Hallucinations in Code Change to Natural Language Generation: Prevalence and Evaluation of Detection Metrics

Language models have shown strong capabilities across a wide range of tasks in software engineering, such as code generation, yet they suffer from hallucinations. While hallucinations have been studied independently in natural language and code generation, their occurrence in tasks involving code changes which have a structurally complex and context-dependent format of code remains largely unexplored. This paper presents the first comprehensive analysis of hallucinations in two critical tasks involving code change to natural language generation: commit message generation and code review comment generation. We quantify the prevalence of hallucinations in recent language models and explore a range of metric-based approaches to automatically detect them. Our findings reveal that approximately 50\% of generated code reviews and 20\% of generated commit messages contain hallucinations. Whilst commonly used metrics are weak detectors on their own, combining multiple metrics substantially improves performance. Notably, model confidence and feature attribution metrics effectively contribute to hallucination detection, showing promise for inference-time detection.\footnote{All code and data will be released upon acceptance.

==> latex/hallucination_detection_techniques_long_version.tex <==
\section{Introduction}
% Large language models (LLMs) have revolutionized many aspects of software engineering, from code generation to documentation tasks. However, these models frequently produce outputs that appear plausible but contain inconsistencies or inaccuracies—a phenomenon known as hallucination. While hallucinations have been extensively studied in general natural language generation and increasingly in code generation, the critical intersection of code-to-natural language generation, particularly in the context of code changes, remains largely unexplored.

% hallucinations of "heterogeneous" data in LLMs

Large language models (LLMs) have revolutionized a wide range of domains and are increasingly being adopted in many real-life workflows. However, these models frequently produce outputs that appear plausible but contain inconsistencies or inaccuracies—a phenomenon known as hallucination.
While this phenomenon exists in unimodal scenarios such as language and visual generation where many prior works have focused, recent studies have found that hallucinations become even more challenging in cross-modality contexts where even the most advanced LLMs struggle due to the representation gaps when translating between different forms of information. 
% recent studies have found that hallucinations become even more challenging in cross-modality contexts where models must translate between different forms of modalities. Even the most advanced LLMs are susceptible to hallucinating in cross-modality generation due to the representation gaps between modalities.
\citet{li-etal-2023-evaluating} demonstrate that large vision-language models consistently hallucinate non-existent objects when generating text descriptions of images due to the transition between visual to text modality.
Interestingly, \citet{sung2024avhbench} found that audio-visual LLMs struggle with hallucinations caused by cross-interactions between modalities, fabricating non-existent sensory inputs across visual and audio domains.


Most recent studies focus on the three modalities: language, visual, and audio.
Yet, little attention has been paid to the hallucinations in code to natural language (NL). On the other hand, while hallucinations have been extensively studied in general natural language generation and increasingly in code generation, the critical intersection of code-to-natural language generation, particularly in the context of code changes, remains largely unexplored.

% While existing research has demonstrated LLMs' capabilities in coding tasks, code summarization, and code review, a critical gap remains in understanding how these models generate potentially misleading descriptions when translating between code and natural language. Unlike single-modal generation tasks, code-to-natural language translation demands simultaneous reasoning across two fundamentally different representational spaces—each with distinct semantic structures and communication norms.



% cross-modality is challenge 
% However, the challenge of hallucinations in code change documentation is further compounded by the inherent difficulty in cross-modality generation. 
 % Even the most advanced LLMs are susceptible to hallucinating in cross-modality generation due to the representation gaps between modalities. Most recent studies focus on the three modalities: language, visual and audio. \citet{li-etal-2023-evaluating} demonstrate that large vision-language models consistently hallucinate non-existent objects when generating text descriptions of images due to the transition between visual to text modality. Interestingly, \citet{sung2024avhbench} found that audio-visual LLMs struggle with hallucinations caused by cross-interactions between modalities, fabricating non-existent sensory inputs across visual and audio domains.

% audio-visual LLMs struggle with hallucinations caused by cross-interactions between modalities, i.e., Audio-visual LLMs tend to hallucinate by perceiving non-existent sounds when presented with visual signals (blue event) or imagining non-existent visual events when given an audio signal (orange event). 
% Yet, little attention has been paid to the hallucinations in code change to NL. 
% or multi-modalities (language, visual, and audio) to text generation \citet{leng2024curse}.
%  \cite{leng2024curse}  first systematic investigation of hallucinations in LMMs involving the three most common modalities: language, visual, and audio.
% \textcolor{red}{why those tasks are important?}
The natural language in code change 
tasks (e.g., code review), serving key communication roles, is often a hybrid of code tokens and human language, which can expose models to the so-called ``curse of crossing modalities``. When attempting to describe or interpret code changes, models must not only understand the code change (or code diff)—an inherently partial view of the entire codebase—but also grasp the underlying semantic intent of those changes. This dual challenge greatly increases the risk of misinterpretation (e.g., developer's intent) and hallucination (e.g., hallucinate the functionality of a piece of code).

% the model needs to effectively bridge two different modalities and avoid generating information not grounded in the input (the code change)

% Similarly, code-to-NL models face a uniquely challenging translation task that demands simultaneous reasoning across two different representational spaces—programming languages and natural language. 
% The NL in code-to-NL tasks are often a mixed of code tokens and natural language, and the generation of the NL means model might also suffer the cross the modalities curse.  When models attempt to describe or understand code change, they must simultaneously comprehend both the code diff—a partial context of a whole repository—and the semantic intent of changes, significantly increasing the risk of misinterpretation and fabrication. 

% consequence of hallucinations in code-diff to NL 
Importantly, accurate communication remains the lifeline of modern software development, while hallucinations in code change documentation critically undermine system reliability and security. 
Especially in a collaborative environment, developers often rely on documentation such as commit messages and code review comments to navigate complex codebases, and therefore clear communication about code changes is crucial. 
However, the growing adoption of AI assistants in software development workflows amplifies the potential impact of hallucinations. When these tools produce plausible but incorrect explanations of code changes, they can (a) mislead developers about the intent and scope of modifications; (b) waste valuable time through misinterpretation; and (c) potentially introduce subtle bugs or security vulnerabilities that evade detection during code review. 



% However, the challenge of hallucinations in code change documentation is further compounded by the inherent difficulty in cross-modality generation \cite{li-etal-2023-evaluating}. Code-to-NL models face a uniquely challenging translation task that demands simultaneous reasoning across two different representational spaces—programming languages and natural language. When models attempt to describe code changes or generate a code review, they must navigate the complex space between precise computational logic and contextual interpretation, transforming a partial repository context into a comprehensible narrative while maintaining the semantic intent of the changes.

% Yet, there is a lack of investigation.

% This translation requires models to simultaneously capture the exact semantic intent of code modifications, translate technical changes into communicative natural languages. 

% The representation gap between structured, deterministic code and ambiguous, context-dependent natural language creates a unique challenge.
%  For instances, models might describe changes that never occurred, misrepresenting actual code modifications, or raising non-existent issues in code reviews. 
% For instance, while a code change might involve a subtle optimization, a model might hallucinate an elaborate motivation that doesn't reflect the actual intent. 
% This misalignment stems from the fundamentally different information encoding in programming languages versus natural language: where code represents precise computational logic, natural language thrives on contextual interpretation and implied meaning.




% why hallucinations detection is difficult? 
% Additionally, another challenge arises from the absence of reliable verification methods. 
% While many hallucination detection techniques have been developed for NL or code, automatic detecting hallucinations in code-diff to natural language tasks presents unique challenges that existing verification approaches cannot adequately address.
Additionally, the absence of reliable verification methods presents another significant challenge in detecting hallucinations in code-diff to natural language tasks.
Unlike code generation, which is often verified through compilation and test execution, or factual text generation, which can be validated against knowledge bases, code change descriptions face two fundamental verification barriers: First, multiple valid descriptions can exist for the same code change, making reference-based evaluation inherently limited. Second, there are no existing knowledge graphs to directly support the verification, or verification requires a significant amount of domain/project-specific knowledge that cannot be easily generalized or automated.


% what's our focus/goal 
In this paper, we address this critical gap by investigating hallucinations in two important code change communication tasks: commit message generation and code review comment generation. We aim to understand the severity of hallucinations in code-diff to natural language tasks and explore automatic detection methods for this increasingly important problem. The two communication tasks represent different ends of the spectrum—commit messages tend to be more descriptive and objective, capturing ``what'' changed and ``why", while code review comments often include subjective assessments and suggestions for issues that cannot be detected using statistic analysis tools. This diversity allows us to explore the full range of hallucination challenges in code-diff to natural language generation. 


% Methdology: How do we reach our goal? 
Our methodology employs a mixed-methods approach combining qualitative analysis and quantitative evaluation. First, we develop a specialized taxonomy for hallucinations in code-diff tasks through systematic annotation of three recent fine-tuned LLMs (Qwen2.5-7b, Llama3.1-8b,CCT5) outputs. This allows us to characterize distinct hallucination types and their prevalence. Second, we evaluate how well existing halluciation detection metrics correlate with these hallucinations, testing both reference-based metrics (BLEU, ROUGE) and reference-free approaches (model uncertainty, semantic similarity). Finally, we introduce a novel feature attribution technique that analyzes how models utilize both changed and unchanged code segments during generation, revealing distinct patterns that can indicate when hallucinations are occurring.


% our contributions 
Our contributions include: (1) a novel decisio-tree like taxonomy specifically designed for hallucinations in code-diff to NL tasks, capturing the unique ways these hallucinations manifest; (2) manually annotated test sets with fine-grained hallucination types that reveal the severity and patterns of the problem; (3) a comprehensive evaluation of existing hallucination detection approaches, demonstrating the limitations of traditional reference-based and reference-free metrics in this domain; and (4) a novel feature attribution approach that analyzes how changed versus unchanged code segments influence text generation, providing insights into model behaviors that indicate hallucination.

This work represents the first systematic investigation of hallucinations in code change communication and provides valuable findings for improving the reliability of AI-assisted software communication tools.

% \section{Introduction}
% % why do we want to do this work? 
% Good and reliable communication is key to many tasks in software development processes, particularly in tasks that require collaborative understanding and sharing, such as documenting and reviewing code changes.
% For example, when developers write commit messages, conveying the intent and implementation details of their changes directly impacts both future team members investigating code history and code reviewers reviewing the code.
% Similarly, reviewers' comments serve as critical feedback that guides code authors in revising their code. These communication tasks, while essential, often require significant manual effort and cause disruptive context switching, ultimately affecting developer productivity~\cite{czerwonka}.


% Recent advances in deep learning and large language models have enabled significant progress in automating these tasks, such as generating code review comments and commit messages.
% While these advances promise to reduce developer burden, they also introduce a critical challenge: hallucination. These models can generate content that appears plausible but contains incorrect content—describing changes that never occurred, misrepresenting actual code modifications, or raising non-existent issues in code reviews. Such inaccuracies not only waste developer time but could also compromise code quality and project understanding. Despite these risks and the growing adoption of AI-assisted tools, there has been limited systematic investigation into hallucination patterns in automated code-change related tasks.



% \begin{color}{red}
% % \textcolor{purple}{%
% many LLMs can do coding tasks, summarization, reviewing the code;
% unique input data,
% no one has ever checked explicitly if the model halluciate or not 
% but this is a more challeing task 
% % note: show challnge:
% % why are we doning code-diff (nl);' why we nned to do this in this contenxt 
% (key problem) 
% need specific domain knowledge 
% good reasoning between the multi-modal (code and text) all, together, could be challenging for LLMs to reason and hallucinate 

% there is a space gap: models have to shift from code space to language space, it's likely that the models are likely will hallu

% the important part is that the NL will be used by SE engineering  
% (if we can show/prove/highlight that hallucinations are more likely to happen in multi-modality than single-modality)
% \end{color}

% % Although progress in developing models on large scale datasets have been made, existing work mainly rely on quality measure metrics such BLEU to measure the quality of generated content. 
% % [how to introduce that models might fabricate content, little work have develed deep into this]


% In this study, we investigate the severity and patterns of hallucination in code change to text generation tasks and study the correlation between existing quality measures and hallucinations.

% % we examine two code change to natural language tasks: code review comment generation and commit message generation. As these tasks are fundamental to modern software development practices and play a crucial role in maintaining software quality and facilitating team collaboration, understanding LLM reliability in generating such content is crucial for their adoption in development workflows. 
% % little attention have been paid on the evaluation of the generated content due to the chall
% % Due to the __  mannual effort

% % the quality of generated text matters,
% % prior work
% % evalaute the correctnedd of code review comments is a difficult thing, there is a lack of automated evaluation metrics to measure the correctness of the generated comments, 

% % In the previour work, when I was doing manul annotation on the quality of the generated comments,
% % I noticed that the some review comments might have a high informative scores based on our definition, but the generated content 




% Our main contributions are: 
% % analysis based work, (1) reveal the degree of hallucination on different types and proportion (2) reveal the capability of automatically detect the halluciations 
% % What's new in this paper? 
% % 
% % what's your baseline? 
% % logic thing: can repeat peanltiy solve the problem already??? 
% \begin{itemize}
%     \item We present the first empirical study that systematically characterizes hallucination patterns in code-diff to text models through a mixed-methods analysis of fine-grained hallucination types.
%     \item Our comprehensive evaluation demonstrates that existing metrics for measuring text quality (both reference-based and reference-free) are inadequate predictors of hallucinations in code-diff scenarios, highlighting the need for specialized evaluation approaches in this domain.
    
%     \item  We introduce a novel hallucination detection method specifically designed for code-diff scenarios that leverages feature attribution to measure how changed and unchanged code segments influence text generation. Our approach achieves X\% improvement in hallucination detection compared to traditional methods. 

% \end{itemize}


\section{Related Work}

% key words: code change to NL tasks, hallucination taxonomy, quality meaures, 
% narrative, the quality of code chagne to  


% how do other people define hallucination
% how do other people detect/quantify hallucination 
% how do other people mitigate hallucination 

\begin{color}{red}
Notes: 

Halluciante in NL only  (definition; scenarios (translation); taxonomy ) 
Halluciante in Code only  (code generation; taxonomy- execute the code to get the results; it's easier to evaluate in the  (we can check syntax or Abstract syntax tree or control flow graph))

no one has done code 2 nl before  (it's harder, cause we cannot use these techniques used in code only) ; we don't know if the techniques used in NL only work in the multi-modal data (context) 

$\rightarrow$ is this true? code summarization is code to nl as well, how is it different from us? or do we research and claim that no one has done this as well?

% \subsection{Code change to natural language generation} 
what people are doing in hallucination;
what can be applied;
what might not be able to apply; (what are the challenges) 
link The automatic quality evaluation metrics

\end{color}

\subsection{Hallucination in code and NL}


\paragraph{Hallucination in Natural Language Generation}
Hallucinations in natural language generation (NLG) tasks have been intensively studied, with taxonomies evolving from simple binary classifications to more fine-grained types that better capture the complexities of recent LLMs. 

Initially, \citet{maynez-etal-2020-faithfulness} categorized hallucinations in abstract summarization into two broad types: \textbf{intrinsic/faithful} hallucinations (where models misinterpret information present in the input, generating content that contradicts the source document) and \textbf{extrinsic/factual} hallucinations (where models forge information absent from the input that cannot be verified using available information). This basic distinction provided a starting point but proved insufficient as LLMs became more sophisticated and widely deployed in various situations.


Previous definitions of intrinsic hallucinations were often task-specific and primarily grounded in the input document \cite{maynez-etal-2020-faithfulness}.
To address the increasingly user-instruction-centric applications of LLMs across various domains, \citet{Huang2025Survey} identified three subcategories of intrinsic hallucinations: instruction-inconsistent (outputs are not consistent with the instruction), logic inconsistency (output itself exhibits internal logical contradictions), context inconsistency (outputs are not consistent with the provided input context). 

Regarding extrinsic hallucinations, researchers discovered that while some content cannot be inferred from the source text, many instances can still be verified against world knowledge \cite{maynez-etal-2020-faithfulness, cao-etal-2022-hallucinated}. Consequently, subsequent research has focused on evaluating outputs classified as extrinsic hallucinations by fact-checking them against world knowledge, labeling those that are factually incorrect as ``factual hallucinations''. \citet{Huang2025Survey} further refined this category by distinguishing between factual contradiction (outputs that can be grounded but contradict with real-world knowledge) and factual fabrication (outputs that are completely made up with no basis in reality or verifiable facts).


% based on \cite{ji2023survey}, 


\paragraph{Hallucination in Code Generation}
A bunch of recent studies have focused on exploring the different types of hallucinations in code generation under different scenarios. % and analyzing their root cause. 

\citet{liu2024exploring} developed a comprehensive taxonomy to classify hallucinations in code generated by LLMs. The taxonomy was established by manually conducting a thematic analysis on 3,084 code snippets generated by various LLMs. The taxonomy includes three high-level types (Intent Conflicting, Context Deviation, and Knowledge conflicting) and 19 subtypes that are code specific (e.g., dead code, using un-imported library). 
This work is based on existing benchmarks (i.e., HumanEval \cite{chen2021evaluating} and DS-1000 \cite{lai2023ds}) for standalone function/script generation instead.
% HALLUCODE: taxonomy, analyzed the distribution, detection, mitigation ; we borrowed some of their types as well (Incon

% \citet{agarwal2024codemirage} define hallucinated code as the generated code that has one or more code defects such as dead or unreachable code, syntactic or logical errors, robustness issues such as the code fails on edge cases or raises an exception, or has security vulnerabilities or memory leaks.
Based on different types of code defects, \citet{agarwal2024codemirage} define five hallucination types (Dead/unreachable code, Syntactic incorrectness, Logical error
Robustness issue, Security vulnerabilities), and introduce CodeMirage dataset based on HumanEval and MBPP to investigate the types of hallucinations in code generated by GPT-3.5. % 
The data was sourced from two existing datasets: HumanEval and MBPP.


\citet{zhang2024llm} studies LLM hallucinations within more practical and complex development contexts in a repository-level generation scenario. They define three broad types (Task Requirement Conflicts, Factual Knowledge Conflicts, Project Context Conflicts) and 8 subtypes. %and also analyzes the root cause of hallucinations.
%have similar structure as ours (taxonomy; llm hallucination pattern and distribution analysis; and root cause analysis; + RAG to mitigate)

Many code generation tasks are executable as well, making it easier to identify potential hallucinations and behavior inconsistency against ground truth. \citet{tian2024codehalu} introduced CodeHalu to detect code hallucinations through actual execution of LLM-generated code against test cases, recording execution errors, and comparing results with expected outputs. Their execution-based verification approach identified four hallucination types (mapping, naming, resource, and logic) by analyzing failure patterns across 17 LLMs, providing concrete evidence of functional correctness issues rather than relying on static code analysis.


\paragraph{Hallucinations in multi-modalities}
% Evaluating Object Hallucination in Large Vision-Language Models ; https://aclanthology.org/2023.emnlp-main.20.pdf 

% Hallucinations in image-to-text (Zhai et al. (2023) three main types of hallucinations: object existence hallucinations, object attribute hallucinations, and object relationship hallucinations.


\subsection{Existing Hallucination Detection Approach}

\subsubsection{referce-based (quality-based)}
\subsubsection{referce-free (uncertainty-based)}

will they work on our context or not 

\paragraph{Feature Attribution for hallucination}
\cite{Snyderetal2024-Early} observed 
distributions of these feature attribution tend  to differ between hallucinated and non-hallucinated generations. They use Integrated Gradient as a feature attribution approach. 

\paragraph{Hallucination detection in code} \cite{agarwal2024codemirage}  explored code hallucination detection with few-shot prompting recent LLMs (GPT-3.5, GPT-4, CodeLLaMA and fine-tuned CodeBERT) and found they often struggle with the automatic detection. 


\subsection{Hallucination Mitigation?}

To mitigate the hallucination problem that models 
 “hallucinate”, or generate non-existent APIs or produce variants of already existing code, \cite{eghbali2024hallucinator} present De-Hallucinator to automatically identify project-specific API references related to the model’s initial predictions and adds these references into the prompt. % less relevant at the moment, but we might want to add some halluciantion mitigation related things later on in future work or limitation 


\textcolor{red}{note: we need to talk about our distinction between errors and hallucinations}


\section{Hallucination Detection Methodology}

We consider both reference-based and reference-free hallucination detection approaches to address different practical needs. Reference-based metrics serve as valuable benchmarks during model training and evaluation when gold standards are available, while reference-free methods enable hallucination detection in real-world deployment scenarios where reference texts are typically unavailable. For example, when code authors use AI to assist the generation of commit messages or code reviewers use AI to assist the generation of code reviews, in-time hallucination detection can help them identify potentially inaccurate content before it's incorporated into the software development process, avoiding miscommunication and reducing technical debt from misleading documentation.

By investigating both approaches simultaneously, we can assess their relative strengths and develop a comprehensive detection framework applicable throughout the entire model lifecycle—from development to production deployment.

\begin{color}{red}
RF-based: This will help during the model training
RF-free: This will help during the model deployment; feature attribution: 

\end{color}

\subsection{Reference-based Metrics}
In reference-based metrics, the quality of a generation $y$ is evaluated by comparing against the reference $\hat{y}$ using a metric. The metric score often indicates the quality of $y$. The hypothesis is that the lower the quality is, the more likely $y$ is a hallucination. Several metrics are widely used: 

% \begin{color}{red}
% RF-based: This will help during the model training
% RF-free: This will help during the model deployment; feature attribution: 

% code to NLP
% code generation 
% NLP to CODE 

% \end{color}

\textbf{Lexical overlap} metrics such as {BLEU}, ROUGE-L and METEOR evaluate the n-gram overlap between the $y$ and $\hat{y}$. This metrics has been widely used in prior work to evaluate the quality of generated commit messages \cite{liu2018neural,li2024only} and review comments \cite{tufano2021towards,Li2022CodeReviewer}. Recently, it has also been adapted to study the correlation with hallucinations in natural language processing tasks, such as neural machine translation \cite{guerreiro-etal-2023-looking,dale-etal-2023-detecting}. 


\textbf{Natural Language Inference (NLI)-based metrics.} NLI is a standard NLP task that determines whether a hypothesis is true (entailment), false
(contradiction), or undetermined (neutral) given a premise.
This has been used to evaluate the factual consistency between a model generation (hypothesis) and a reference (premise) \cite{hu2024refchecker, valentin2024cost}. 
The $y$ is considered as a premise and $\hat{y}$ is the hypothesis, if the $y$ can be  directly inferred from the reference $\hat{y}$, an entailment relationship holds.  Conversely, if it contradicts the information in the reference, it is labeled as
contradiction. In cases where the reference is insufficient to verify the $y$, it is classified as Neutral.
Commonly used NLI models including Align Score (Zha et al., 2023) and RoBERTa-NLI. However, these models are mostly trained on natural languages only, its suitability to commit message or code review comments which contain both natural language and code tokens needs further exploration. 
While NLI has been used in sampling-based approaches for hallucination detection to assess factual consistency \cite{manakul-etal-2023-selfcheckgpt, elaraby2023halo}, these methods typically involve quantifying the consistency of NLI relationships across multiple generations. In our situation, we only consider the relationship between the $\hat{y}$ and a single generation $y$. 


% \textbf{Embedding Similarity} measures the distance of two pieces of inputs, e.g., a generation $y$ and its reference $\hat{y}$. Typically, the sentence embeddings of model generation and its reference are extracted using an embedding model and cosine similarity is applied to estimate the distance \cite{chen2024inside,sanayei-etal-2024-maria, huang2023look}. 

% \cite{dale-etal-2023-detecting} 

\subsection{Reference-free Metrics}
We use reference-free metrics that either use information from the source input or from the model behaviors while generating a sequence. 

% The generator is defined as the model used to generate the original response. The detector LLM is the model used to score a generated text for the presence of hallucinations. 
\subsubsection{Similarity between the generation and the source}
Different from the reference-based embedding similarity, here we consider the  semantic distance between the source and the generation. 

\subsubsection{Sequence-level confidence scores}
A sequence-level confidence score is calculated via aggregating token-level uncertainty into sentence level by taking the average across the sequence. % or max
Token-level confidence can be measured in various ways. The hypothesis is when model hallucinates, it tend to be less confident. 
Several metrics have been proposed to estimate the token-level uncertainty, including probability, logit and entropy \cite{guerreiro-etal-2023-looking,huang2023look, valentin2024cost}. The length-normalized sequence log-probability (\textbf{SeqLogProb}): 
\begin{align}
    \label{eq:seqlogprob}
    \text{SeqLogProb} = \frac{1}{L}\sum_{t=1}^{L} - \log{p_t},
\end{align}
where the $p_t$ is the probability of generating a token at position $t$, $L$ is the total length of the sequence. 
% note: perplexity takes a exp() outside the seqlogprob

Likewise, the raw logit before Softmax-normalization can also be used be estimate the uncertainty of generating a token $y_t$, where smaller raw logit indicate less confident. We name this approach  \textbf{SeqLogit}, which can be formulated as: 
\begin{align}
    \label{eq:seqlogit}
    \text{SeqLogit} = \frac{1}{L}\sum_{i=1}^{L} {\text{Logit}_t},
\end{align}

Furthermore, when generating a token, the confidence can also be measured by the entropy of the token distribution. When the token distribution is more uniform across the vocabulary, the model tend to be less certain about its generation. This can be formulated as follows: 
% \textbf{SeqEntropy}
\begin{align}
    \label{eq:seqeng}
    \text{SeqEntropy} = \frac{1}{L}\sum_{i=1}^{L} {H_i},
\end{align}
where $H_i$ is the entropy of the token distribution. A higher $H_i$ indicates the more uncertain the model is about the generation. 

\subsubsection{Feature Attribution.}  
Given an input $x \in \mathbb{R}^n$ where $x_i \in \mathbb{R}^d$, a model generates a token $y_i$ at each time step. Feature attribution methods assign to each $x_1, x_2, ..., x_n$ attribution values $A(x_1), A(x_2), ..., A(x_n)$, indicating their contributions to generating $y_t$. Using feature attribution, we obtain a matrix $A \in \mathbb{R}^{n \times T}$, representing the attribution value of each input token to each output token. To investigate hallucinations, we apply an aggregation function on $A$ to convert it into a single sequence of attribution values.

We employ two widely used feature attribution methods: Saliency~\cite{simonyan2014deepinsideconvolutionalnetworks} and Input X Gradient~\cite{pmlr-v70-shrikumar17a}. The Saliency method calculates the gradient of output with respect to input:

\begin{align}
A_{i,t} = \frac{\partial y_t}{\partial x_i}    
\end{align}

where $A_{i,t}$ represents the attribution score of input token $x_i$ for output token $y_t$. The gradient indicates how sensitive the output is to changes in each input token. However, Saliency only considers gradients, potentially overlooking the impact of input magnitudes on generation. To address this limitation, Input X Gradient extends the approach by incorporating input magnitudes:

\begin{align}
    A_{i,t} = x_i \times \frac{\partial y_t}{\partial x_i}
\end{align}

This method accounts for both gradient sensitivity and actual input values $x_i$, providing attribution scores that reflect both the model's responsiveness to input changes and the scale of the inputs themselves.


\textbf{Attribution Aggregation.} To obtain a single attribution score for the sequence, we first compute the maximum attribution value across all input tokens for each output token $y_t$, then take the average of these maximum values:
\begin{align}
    \text{SourceAttr} = \frac{1}{T}\sum_{t=1}^{T} \max_{i \in [1,N]} A_{i,t},
\end{align}

where $\text{SourceAttr}$ represents final sequence-level overall source contribution score. The hypothesis is when the maximum input contribution is small, 
the generated $y$ is likely to be a hallucination as the model didn't generate based on the input. 

Given our input is a code change consisting of both old and new code, human developers primarily focus on the changed parts when generating commit messages and code review comments. Based on this observation and the assumption that models should similarly emphasize code changes, we designed variations of the aggregation methods that separate attribution scores for changed and unchanged code. Our hypothesis is that lower attribution scores on the changed parts indicate a higher likelihood of hallucination.
\begin{align}
    \text{ChangedAttr} &= \frac{1}{T}\sum_{t=1}^{T} \max_{i \in C} A_{i,t}, \\
    \text{UnchangedAttr} &= \frac{1}{T}\sum_{t=1}^{T} \max_{i \in [1,N] \setminus C} A_{i,t}, \\
    \rho = \frac{\text{ChangedAttr}}{\text{UnchangedAttr}}
\end{align}
where $C \subset [1,N]$ represents the indices of tokens in the changed code (all - and + lines), and $[1,N] \setminus C$ represents the indices of unchanged code tokens.
\textcolor{red}{We also calculated the ratio of changed attrition score to the unchanged attribution score, a higher ratio indicate that more contribution from changed part than unchanged part. }

==> latex/tables/top_individual_metrics_codereviewer.tex <==



\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{|c|l|c|}
\hline
\textbf{Rank} & \textbf{Metric} & \textbf{Score} \\
\midrule
\multicolumn{3}{|c|}{Top 5 by ROC-AUC} \\ 
\midrule 
1 & logit\_Llama3.1 & 0.566 \\
2 & entropy\_CCT5 & 0.560 \\
3 & entropy\_Qwen2.5 & 0.552 \\
4 & logit\_Qwen2.5 & 0.548 \\
5 & similarity\_score\_codebert-base & 0.538 \\
\midrule 
\multicolumn{3}{|c|}{Top 5 by |Point-Biserial|} \\ 
\midrule 
1 & BLEU & -0.155 \\
2 & entailment\_score & -0.119 \\
3 & source\_target\_contrib\_Llama3.1 & -0.115 \\
4 & logit\_Llama3.1 & 0.076 \\
5 & unchanged\_contribution\_Llama3.1 & -0.06 \\
\bottomrule
\end{tabular}
\caption{Top metrics for hallucination detection across generators on CodeReviewer.}
\label{tab:individual_metrics_overall_hallucination_codereviewer}
\end{table}



\begin{table*}[t]
\scriptsize
\centering
% \renewcommand{\arraystretch}{0.8}
\begin{tabular}{l|l|c|l|c|l|c}
\toprule
Rank & \multicolumn{2}{c}{CCT5} & \multicolumn{2}{c}{Llama3.1} & \multicolumn{2}{c}{Qwen2.5} \\
 % & Metric & roc\_auc & Metric & roc\_auc & Metric & roc\_auc \\
\midrule 
 \multicolumn{7}{c}{\textbf{Top 5 by ROC AUC}} \\
\midrule
1 & logit\_Llama3.1 & 0.71 & source\_target\_contrib\_Llama3.1 & 0.62 & entropy\_CCT5 & 0.67 \\
2 & logit\_Qwen2.5 & 0.68 & source\_target\_contrib\_Qwen2.5 & 0.61 & entropy\_Qwen2.5 & 0.65 \\
3 & logit\_CCT5     & 0.66 & entropy\_Qwen2.5 & 0.58 & entropy\_Llama3.1 & 0.63 \\
4 & prob\_Llama3.1 &  0.66 & entropy\_Llama3.1 & 0.57 & unchanged\_contrib\_Qwen2.5 & 0.59 \\
5 & prob\_Qwen2.5 & 0.65 & unchanged\_contribution\_CCT5 & 0.57 & source\_target\_contrib\_Qwen2.5 & 0.59 \\ 
\midrule
\multicolumn{7}{c}{\textbf{Top 5 by |Point-Biserial Correlation|}} \\ \midrule 
1 & source\_target\_contrib\_Llama3.1 & -0.27 & entailment\_score & -0.19 & BLEU & -0.26 \\
2 & unchanged\_contrib\_Llama3.1 & -0.24 & source\_target\_contrib\_Qwen2.5 & 0.16 & probability\_CCT5 & -0.23 \\
3 & logit\_Llama3.1 & 0.24 & source\_target\_contrib\_Llama3.1 & 0.16 & entropy\_CCT5 & 0.22 \\
4 & similarity\_codet5p-220m-bim & 0.21 & changed\_contri\_Llama3.1 & -0.13 & entropy\_Qwen2.5 & 0.22 \\
5 & prob\_Llama3.1 & 0.20 & target\_target\_contrib\_Qwen2.5 & 0.11 & entropy\_Llama3.1 & 0.20 \\
\bottomrule
\end{tabular}
\raggedright
\small{Note: Higher ROC AUC and larger absolute correlation values indicate better hallucination detection capability.}
\caption{Top 5 metrics for hallucination detection by model on CodeReviewer dataset}
\label{tab:top_individual_metrics_codereviewer}
\end{table*}


==> latex/tables/top_individual_metrics_commitbench.tex <==

\begin{table}[tbp]
\scriptsize
\centering
\begin{tabular}{|c|l|c|}
\hline
\textbf{Rank} & \textbf{Metric} & \textbf{Score} \\
\midrule
\multicolumn{3}{|c|}{Top 5 by ROC-AUC} \\ 
\midrule 
1 & similarity\_score\_codet5p-770m & 0.617 \\
2 & target\_target\_contrib\_CCT5 & 0.610 \\
3 & logit\_Llama3.1 & 0.600 \\
4 & similarity\_score\_codebert-base & 0.592 \\
5 & logit\_Qwen2.5 & 0.562 \\
\midrule 
\multicolumn{3}{|c|}{Top 5 by |Point-Biserial|} \\ 
\midrule 
1 & BLEU & -0.199 \\
2 & target\_target\_contrib\_CCT5 & 0.173 \\
3 & entailment\_score & -0.164 \\
4 & similarity\_score\_codet5p-770m & 0.152 \\
5 & changed\_contribution\_CCT5 & -0.150 \\
\bottomrule
\end{tabular}
\caption{Top metrics for hallucination detection across generators on CommitBench Dataset}
\label{tab:individual_metrics_overall_hallucination_commitbench}
\end{table}

\begin{table*}[t]
\scriptsize 
\centering
% \renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|l|c|l|c|l|c}
\toprule
\textbf{Rank} & \multicolumn{2}{c|}{\textbf{CCT5}} & \multicolumn{2}{c|}{\textbf{Llama3.1}} & \multicolumn{2}{c}{\textbf{Qwen2.5}} \\
\midrule 
\multicolumn{7}{c}{\textbf{Top 5 by ROC AUC}} \\
\midrule 
1 & target\_target\_contrib\_CCT5 & 0.61 & similarity\_score\_codet5p-770m & 0.68 & logit\_Llama3.1 & 0.63 \\
2 & similarity\_score\_codet5p-770m & 0.58 & similarity\_score\_codebert-base & 0.67 & logit\_Qwen2.5 & 0.60 \\
3 & changed\_contribution\_Qwen2.5 & 0.57 & logit\_Llama3.1 & 0.66 & similarity\_score\_codet5p-770m & 0.58 \\
4 & entropy\_Qwen2.5 & 0.56 & target\_target\_contrib\_CCT5 & 0.63 & target\_target\_contrib\_CCT5 & 0.58 \\
5 & changed\_contribution\_Llama3.1 & 0.56 & logit\_Qwen2.5 & 0.62 & similarity\_score\_codebert-base & 0.58 \\
\midrule 
\multicolumn{7}{c}{\textbf{Top 5 by |Point-Biserial Correlation|}} \\
\midrule 
1 & changed\_contribution\_CCT5 & -0.17 & similarity\_score\_codebert-base & 0.26 & BLEU & -0.21 \\
2 & BLEU & -0.15 & BLEU & -0.25 & logit\_Llama3.1 & 0.18 \\
3 & target\_target\_contrib\_CCT5 & 0.15 & logit\_Llama3.1 & 0.24 & logit\_Qwen2.5 & 0.14 \\
4 & entailment\_score & -0.13 & target\_target\_contrib\_CCT5 & 0.24 & entailment\_score & -0.14 \\
5 & prob\_Qwen2.5 & -0.10 & similarity\_score\_codet5p-770m & 0.24 & similarity\_score\_codebert-base & 0.12 \\
\bottomrule
\end{tabular}
\raggedright
\small{Note: Higher ROC AUC and larger absolute correlation values indicate better hallucination detection capability.}
\caption{Top 5 metrics for hallucination detection by model on CommitBench dataset}
\label{tab:top_individual_metrics_commitbench}
\end{table*}

